Nash Social Welfare for 2-value Instances

This paper is merged with arXiv:2107.08965v2. We refer the reader to the full and updated version. We study the problem of allocating a set of indivisible goods among agents with 2-value additive valuations. Our goal is to find an allocation with maximum Nash social welfare, i.e., the geometric mean of the valuations of the agents. We give a polynomial-time algorithm to find a Nash social welfare maximizing allocation when the valuation functions are integrally 2-valued, i.e., each agent has a value either $1$ or $p$ for each good, for some positive integer $p$. We then extend our algorithm to find a better approximation factor for general 2-value instances.

==> Half-integer.tex <==
 
\section{Half-integer p}

In this section we consider that agents have arbitrary valuations and $2p \in \mathbb{N}$.

\begin{lemma}
    Let $A^*$ be the allocation with maximum NSW and $(u_1(A^*_1), ... , u_n(A^*_n))$ be its utility profile. Then there exists an index $t \in [n]$ such that for all $1 \leq i \leq t$: $u_i(A^*) = u_1 + \{0, 0.5, 1\}$ and for all $i > t: u_i(A^*) = kp > u_1(A^*) + 1$ for some $k \in \mathbb{N}$. 
\end{lemma}

\begin{proof}
    The allocation of light goods is greedy and $t = \max(\{i \in [n], u_i(A^*_i) \in u_1(A^*_1)+\{0, 0.5, 1\})$.
\end{proof}

\begin{lemma}
    Let $X$ be an allocation  such that for all $i \in N$, $u_i(X_i) = u_1(X_1) + \{0, 0.5, 1\}$. Then among all allocations with the same number of heavy goods as X, an allocation $A^*$ maximizes NSW if and only if for all $i \in N$, $u_i(A^*) = u_1(X) + \{ 0, 0.5, 1\}$ and $|\{i \in N | u_i(A^*) = u_1(X_1) + 0.5\}|$ is maximum.
\end{lemma}

\begin{proof}
    \Red{TODO}
\end{proof}

Note that the parity of the number of heavy goods in $X_i$ in which $u_i(X_i) = u_1(X_1) + \{ 0.5\}$ is different from the parity of the number of heavy goods in $X_j$ in which $u_j(X_j) = u_1(X_1) + \{0\}$ and $X_k$ in which $u_k(X_k) = u_1(X_1) + \{ 1\}$. We called the parity of the number of heavy goods in $X_i$, right parity.


Consider a bipartite graph $G= (N \cup M, E)$, in which vertices in one part represent agents and vertices in another part represent goods.
We have an edge between the agent $a_i$ and the good $g_j$ if $v_i(g_j) = p$.
So, we want to find a maximum multi matching in this bipartite graph which maximizes the number of agents with right parity.
\begin{definition}
    Augmenting Path. We call a path between two agents an augmenting path if for all odd $i \in [n]$, exactly one of the $i_{th}$ and $i+1_{th}$ edges belong to the maximum multi matching.
\end{definition}


\begin{algorithm}
    \caption{GoodMatching} \label{goodmatching}
    %Input: $N, M,  u = (u_1, ... , u_n), B = (B_1, ... , B_n)$ 
    Input: $G$, Maximum multi matching $\mathcal{M}$
    Output: $C = (C_1, ..., C_n)$
    
    \begin{algorithmic}[1]
        
        \While {there are two agents with wrong parity in $\mathcal{M} $ and an Augmenting path between them}
            \State unmatch every matched edge and simultaneously match every unmatched edge
        \EndWhile
        
        \State return $C$
    \end{algorithmic}
\end{algorithm}


\begin{definition}
    Distance of two multi matching. Number of agents with different parity in these two multi matching.
\end{definition}

\begin{lemma}
    Algorithm ~\ref{goodmatching} gives us a maximum multi-matching with maximum number of agents with right parity.
\end{lemma}
\begin{proof}
    Let $OPT$ be an optimum multi matching with minimum distance with $C$. Consider the bipartite graph $G' = OPT \cup C$. Remove all cycles of length two to obtain a simple bipartite graph. All goods have an even degree. Agents with the same parity in $OPT$ and $C$ have an even degree and agents with different parity in $OPT$ and $C$ have an odd degree. 
    Remove all cycles. The parities of degrees do not change. Consider the longest path. The first and last vertices in this path have an odd degree, which means they have different parity in $OPT$ and $C$. We can assume that both have wrong parity in $C$ because otherwise, $OPT$ does not have minimum distance with $C$. This leads us to a contradiction because we have an augmenting path between two vertices with wrong parity in $C$.
    
   Therefore after removing all cycles, we do not have any path. Hence, we do not have any vertex with an odd degree and we can conclude that the number of agents with the right parity in $OPT$ and $C$ are the same.
    
\end{proof}



\begin{algorithm}
    \caption{NSWsmallAgents}
    Input: $N, M,  u = (u_1, ... , u_n), B = (B_1, ... , B_n)$ 
    
    Output: $C = (C_1, ..., C_n)$
    
    \begin{algorithmic}[1]
    
        \State sort agents such that $u_1(B_1) \leq ... \leq u_n(B_n)$
        \State let $t+1$ be the minimum index s.t. $u_{t+1}(B_{t+1}) > u_1(B_1) + 1$

        \State $\mu = \frac{1}{t} (\Sigma_{i=1}^{t} u_i(B_i))$
        \State let $M'$ be the set of all items that assigned to the first $t$ agents
        
        \State $C[t .. n] = B[t .. n]$
        \State $C[0 .. t] = argmax\{NSW(GoodMatching([t], M',u[0 .. t], \ceil{\mu})), \newline NSW(GoodMatching([t], M', u[0 .. t], \ceil{\mu} + 0.5))\}$
        
        \State return $C$
    \end{algorithmic}
\end{algorithm}

\begin{algorithm}
    \caption{HalfInteger} \label{halfintalg}
    Input : $N, M, u = (u_1, ... , u_n)$ 
    
    Output: allocation $B = (B_1, ... , B_n)$
    \begin{algorithmic}[1]
    
        \State $u'_i = \floor{u_i / p}$
        \State $B = $BinaryMaxNSW$(N, M, u')$
        
        \While {there is an unallocated item $g$}
            \State let $u_1(B_1) \le u_2(B_2) \le ... \le u_n(B_n)$
            \State $B_1 \leftarrow B_1 \cup \{g\}$
        \EndWhile        
        \State $B \leftarrow NSWsmallAgents(N, M, u, B)$
        \While{$(u_1(B_1) + 1) / u_n(B_n) < 1/p$}
            \State $B_n \leftarrow B_n \backslash \{g\}$
            \State $B_1 \leftarrow B_1 \cup \{g\}$
            \State $B \leftarrow NSWsmallAgents(N, M, u, B)$
        \EndWhile
        \State return $B$
    \end{algorithmic}
\end{algorithm}


==> Identical.tex <==
 \section{Identical valuations, rational p}
 
 Consider a 2-valued instance $(N, M, \uv)$ with identical valuations. Let w.l.o.g $1 \leq p = \frac a b$ the two possible valuations. Consider $G = H \sqcup L$ the partition of $G$ into heavy and light goods. Let $h = \abs H$ and $l = \abs L$.
 
 In order to maximize the $\NSW$, we are only interested in the number of heavy and light goods each agent is allocated. Thus, we search for $h$ and $l \in (\mathbb Z_{\leq 0})^N$ such that:\begin{itemize}
     \item $\sum\limits_{i \in N} h_i = h$
     \item $\sum\limits_{i \in N} l_i = l$
     \item $\prod\limits_{i \in A} ph_i+l_i$ is maximized.
 \end{itemize}
 
 \begin{lemma} There exists $h$ and $l$ satisfying the above conditions and such that: \[\forall i, j \in A, \abs{h_i-h_j} \leq b\] \end{lemma}
 
 \begin{proof} Assume that we have $i, j \in N$ such that $h_j \geq h_i+b+1$. Let $v_i = (ph_i + l_i)_{i \in N}$. For $x, y \in \mathbb R$ and $d \in \mathbb R_{>0}$, we have:\[\begin{array}{rcl}
 xy \leq (x-d)(y+d)&\Leftrightarrow&d \leq x-y\end{array}\]
 \begin{itemize}
     \item If $p \leq \uv_j - \uv_i$ then setting $h_i \assign h_i+1$ and $h_j \assign h_j-1$ does not reduce the $\NSW$ and increases $h$ on the leximin front
     \item If $\uv_j \leq \uv_i+p$, then $l_i \geq l_i-l_j \geq p(h_j-h_i-1) \geq bp$ and setting \begin{itemize}
         \item $h_i \assign h_i+b$
         \item $h_j \assign h_j-b$
         \item $l_i \assign l_i-bp$
         \item $l_j \assign l_j+bp$
     \end{itemize}
     Does not change change $\uv_i$ and $\uv_j$ and increases $h$ on the leximin front
 \end{itemize}
 
 In any case, $h$ is not leximin among all vectors such that there exists $l$ satisfying the conditions.
 \end{proof}
 
 For $h \in (\mathbb Z_{\leq 0})^N$, let $Greedy(h) \in (\mathbb Z_{\leq 0})^N$ be the vector giving, for each agent, the number of light goods he receives in the greedy allocation.
 
 The problem is now to find $h \in \underset{\substack{h \in (\mathbb Z_{\leq 0})^N\\\sum\limits_{i \in N} h_i = h\\\forall i, j \in N, \abs{h_i-h_j} \leq b}}{\text{argmax}} \prod\limits_{i \in A} h_i p + Greedy(h)_i$.
 
 \begin{lemma} 
 Let $h$ verifying the preceding lemma. Then $im(h) \subset \lbracket \ceil{\frac h n} - b, \floor{\frac h n}+b \rrbracket$. \KM{$\mathit{im}(h) \subseteq \left[ \ceil{\frac{h}{n}} - b, \floor{\frac{h}{n}} + b\right]$.} \KM{im: If you write $im$, TeX believes that you mean the product of $i$ and $m$. But you mean a function name. Then it should be $\mathit{im}$. This looks almost the same. But here comes an example where you see the difference: $diff$ versus $\mathit{diff}$}.
 \end{lemma}
 
 \begin{proof} Let $x = \min\limits_{i \in A} h_i$. Then $h = \sum\limits_{i \in A} h_i \leq n(x+b)$. Thus $\frac h n - b \leq x$. As $x$ and $b$ are integers, $\ceil{\frac h n} - b \leq x$
 
 Let $X = \max\limits_{i \in N} h_i$. Then $n(X-b) \leq \sum\limits_{i \in N} h_i \leq h$. Thus $X \leq \frac h n + b$. As $X$ and $b$ are integers, $X \leq \floor{\frac h n} + b$. \end{proof}
 
 Up to giving on order on $N$ such that $h$ is non decreasing, giving $h$ is equivalent to giving $(\abs{\{i \in N, h_i = x\}})_{x \in \mathbb Z_{\leq 0}}$. We have a bijection between \[\{h \in (\mathbb Z_{\leq 0})^N, h \nearrow \land \sum\limits_{i \in N} h_i = h \land \forall i, j \in N, \abs{h_i-h_j} \leq b\}\] and \[\bigcup\limits_{a \in \llbracket \ceil{\frac h n} - b, \ceil{\frac h n} \rrbracket} \{x \in (\mathbb Z
^+)^{\llbracket a, a+b}, \sum\limits_{a \leq i \leq a+b} x_i = n \land \sum\limits_{a \leq i \leq a+b} i x_i = h\}\]

Furthermore, we have, for $a \in \llbracket \ceil{\frac h n} - b, \ceil{\frac h n} \rrbracket$,\\\[\abs{\{x \in (\mathbb Z
^+)^{\llbracket a, a+b \rrbracket}, \sum\limits_{a \leq i \leq a+b} x_i = n \land \sum\limits_{a \leq i \leq a+b} i x_i = h\}} \leq {n+b \choose b} \underset{n \to +\infty} = O(n^b)\]

==> runtime.tex <==

    \begin{theorem}
        Algorithm \ref{alg2} is polynomial-time.
    \end{theorem}
    \begin{proof}
        In \cite{barman2018greedy}, it is shown that Algorithm \ref{alg1} is polynomial time. Therefore the first phase of the algorithm takes polynomial time. 
    \end{proof}	
    	
	\begin{theorem}
		Runtime of Algorithm \ref{alg1} is $O((n+m)^3m^2)$.
	\end{theorem}
\iffalse
	\begin{proof}
		In this proof, we consider that the graphs are represented via matrices. Constructing $G$ takes time $O((n+m)^2)$. Finding $Q$ takes time $O(nm)$ as one can simply allocate each good to an agent that has utility $1$ for it (if one such agent exists). The last for loop takes time $O(nm)$.
		
		Each round of the while loop takes time $O((n+m)^3)$: consider an allocation $A$ at the start of the while loop. Let $G'$ the graph obtained from $G$ by removing the (directed) edges from $Q$. This construction takes time $O((n+m)^2)$. An alternating path such as described in the algorithm is a path in $G'$. Computing the distance between any two nodes takes time $O((n+m)^3)$, using for example Floyd-Warshall algorithm. Finding a simple alternating path takes time $O(n^3)$ using the distances. Finally, updating $Q$ takes time $O(n)$.
		
		There are $O(m^2)$ rounds of the while loop. To show this, consider $A_0$ the initial allocation and $A_1, ..., A_k$ a sequence of allocations obtained after each iteration of the loop starting with $A_0$. Let $p \in \{0, ...,  k-1\}$ and $i, j \in N$ such that $\abs{A_{p+1}(i)} = \abs{A_p(i)}+1$ and $\abs{A_{p+1}(j)} = \abs{A_p(j)}-1$. $i$ and $j$ are selected such that $\abs{A_p(i)} \leq \abs{A_p(j)}-2$ and the number of goods allocated to any other agent has not changed. We have:\[\begin{array}{rcl}
		||(\abs{A_{p+1}(i)})_{i \in N}||_2^2-||(\abs{A_p(i)})_{i \in N}||_2^2&=&\sum\limits_{i \in N} \abs{A_{p+1}(i)}^2 - \sum\limits_{i \in N} \abs{A_p(i)}^2\\
		&=&\abs{A_{p+1}(i)}^2+\abs{A_{p+1}(j)}^2-\abs{A_p(i)}^2-\abs{A_p(j)}^2\\
		&=&\abs{A_p(i)+1}^2+\abs{A_p(j)-1}^2-\abs{A_p(i)}^2-\abs{A_p(j)}\\
		&=&2(\abs{A_p(i)}-\abs{A_p(j)}+1)\\
		&\leq&-2\end{array}\]
		Now, consider $x: N \to \mathbb R^+$ and $y \in \mathbb R^+$ such that $\sum\limits_{i \in A} x_i = y$. If there are $i \neq j \in N$ such that $0 \notin \{x_i, x_j\}$, replacing $x_i$ and $x_j$ by $x_i+x_j$ and $0$ increases $||x||_2$ (as $x_i^2+x_j^2 \leq (x_i+x_j)^2$). Thus, $\max\limits_{\substack{x: N \to \mathbb R^+\\\sum\limits_{i \in A} x_i = y}} ||x||_2^2 = y^2$. Applying this to our the sequence on allocations, we have $0 \leq ||(\abs{A_k(i)})_{i \in N}||_2^2 \leq ||(\abs{A_0(i)})_{i \in N}||_2^2-2k \leq \abs Q^2-2k$. Thus $k \leq \frac 1 2 m^2$. 
		\end{proof}
\fi
	
	
	

Consider a bipartite graph with the agents on one side and the goods on the other side. There is an edge between an agent and a good if the good can be allocated to the agent. Let $E$ be the set of edges. We represent an allocation by directing the edges.
If a good is allocated to an agent, we direct the edge from the good to the agent. If a good is not allocated to an agent, we direct the edge from the agent to the good.

The indegree of an agent is the size of its bundle. An alternating path from an agent to an agent is simply a directed path from an agent to an agent in this graph.

We can improve NSW as long as there is a directed path where the indegree of the endpoint is at least two larger than the indegree of the starting point. Augmenting the path is tantamount to reversing the direction of all edges on the path.

Suppose now that we always search for augmenting paths starting from a vertex of minimum indegree. If we find an alternating path ending in a vertex whose indegree is as least two larger, we augment. Searching for a path takes time $O(m)$. We can use depth-first search.

Assume now that no such path exists and let $S$ be the set of agents and goods reached in the search, say the search started in $s$. Then there can be no edge leaving the set $S$, i.e., if $\sset{a,g} \in E$ and

$a \in S$ and $g \not\in S$, then the edge is directed from $g$ to $a$, i.e., $g$ is allocated to $a$.

$a \not\in S$ and $g \in S$, then the edge is directed from $a$ to $g$, i.e., $g$ is not allocated to $a$.

So we have
\begin{itemize}
\item The size of the bundles of the agents in $S$ differ by at most one. This holds since $s$ has a minimum size bundle and we do not reach a bundle which is two larger.
\item Every good in $S$ is allocated to an agent in $S$. If a good is reached by the search, the search also reaches the agent to which the good is assigned. 
\item Every good not in $S$ that could potentially be allocated to an agent in $S$, is allocated to an agent in $S$. Otherwise, we would add the good to $S$. 
\end{itemize}
We conclude that the maximum number of goods that can potentially be allocated to the agents in $S$ are allocated to the agents in $S$. Moreover, the size of the bundles are equal up to one. So the allocation is NSW.

We remove the agents in $S$ and the goods allocated to them and repeat.

\begin{theorem} \label{Poly-time}
The running time of the algorithm is $O((n + m) m )$. \end{theorem}
\begin{proof} 
In each round we either increase the size of the bundle of a vertex of minimum bundle size or we remove an agent. There can be at most $n$ iterations of the latter kind. There can be at most $O(m)$ iterations of the former kind. This can be seen as follows. The size of the bundle of a vertex can be increased at most as many times as the final size of the bundle. When the agent is removed, we also remove all goods assigned to him. So the total number of times that we can increase a bundle size is $m$.

  Each round takes $O(m)$  time.
  \end{proof}
  
  Note that the proof also gives us a decomposition of the agents into groups. 
  
  Bundle size min, min +1 and all goods that can possibly be allocated to them. 
  
  Bundle size min+1, min+2 and all remaining goods that can possibly be allocated to them. 
  
  Bundle size min + 2, min +3 and all remaining goods than can possibly be allocated to them. 
  
  I remember that we talked about such a decomposition once in my office but never formalized it. 




